Present Aspects and Future Prospects of Neutrino Mass and Oscillation

Neutrinos are neutral, spin-$\frac{1}{2}$ particles which undergo only weak interactions. The experimentally observed phenomenon of neutrino oscillation establishes the fact that neutrinos are massive and there is mixing between different neutrino flavours. This constitutes the first unambiguous hint towards the physics Beyond Standard Model (BSM). In the BSM theories, the neutrino mass terms in the Lagrangian lead to the non-diagonal neutrino mass matrix in the flavour basis which depends on neutrino mass and mixing parameters. Thus knowledge of the neutrino oscillation parameters and understanding the underlying symmetries of the neutrino mass matrix are very important as they can give an insight to the new physics beyond Standard Model. Therefore the measurement of different oscillation parameters and studying the structure of the neutrino mass matrix are some of the main goals in neutrino physics at present. In this thesis we have studied the potential of present/future neutrino oscillation experiments and synergy between them to determine the unknown parameters in the neutrino sector in the light of current experimental results. We have also studied the phenomenological consequences of texture zeros in the neutrino mass matrices in the presence of a sterile neutrino.

==> abbreviations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%              List  of  Abbreviations               %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 {\Large \textbf{List of Abbreviations}}
\vspace{0.5cm}

\begin{table}[h]
    \begin{center}
    \begin{tabular}{ll}
          BSM         & Beyond Standard Model \\
          SM          & Standard Model \\
          CC          & Charge Current Interaction \\
          NC          & Neutral Current Interaction \\
          LEP         & Large Electron-Positron collider \\
          VEV         & Vacuum Expectation Value \\
          PMNS        & Pontecorvo Maki Nakagawa Sakata Matrix \\
   $0\nu\beta\beta$   & Neutrinoless Double Beta Decay \\
          SSM         & Standard Solar Model \\
          SK          & Super-Kamiokande Experiment \\
          DAR         & Decay at Rest \\
           DIF         & Decay in Flight \\
           IBD         & Inverse Beta Decay \\
           UHE         & Ultra High Energy \\
           AGN         & Active Galactic Nuclei \\
           GRB         & Gamma Ray Burst \\
           GUT         & Grand Unified Theories \\
           NSI         & Non Standard Interaction \\          
           OMSD        & One Mass Scale Dominance Approximation \\
           MSW         & Mikheyev Smirnov Wolfenstein Effect \\
           PREM        & Preliminary Reference Earth Model \\
           GLoBES      & General Long Baseline Experiment Simulator \\
           NH          & Normal Hierarchy \\
           IH          & Inverted Hierarchy \\
            QD          & Quasi-Degenerate \\
%            LO          & Lower Octant \\
%            HO          & Higher Octant \\
%            LHP         & Lower Half Plane of $\dcp$ \\
%            UHP         & Upper Half Plane of $\dcp$ \\
%            T2K         & Tokai to Kamioka \\
%            POT         & Protons on Target \\
%            \nova\      & NuMI Off-axis $\nu_e$ Appearance \\
%            LAGUNA      & Large Apparatus studying Grand Unification and \\
%                        &  Neutrino Astrophysics \\
%            LBNO        & Long Baseline Neutrino Oscillation Experiment\\
%            LBNE        & Long Baseline Neutrino Experiment \\
%            LArTPC      & Liquid Argon Time Projection Chamber \\
%            SURF        & Sanford Underground Research Facility \\
%            DUNE        & Deep Underground Neutrino Experiment \\
%            INO         & India-based Neutrino Observatory \\
%            ICAL        & Iron Calorimeter Detector \\
%            LBL         & Long Baseline Experiments \\
%            CPV         & CP Violation \\
          
         
    \end{tabular}
    \end{center}
\end{table}

\pagebreak
%{\Large \textbf{List of Abbreviations}}
%\vspace{0.5cm}

\begin{table}[h]
    \begin{center}
    \begin{tabular}{ll}
%          BSM         & Beyond Standard Model \\
%          SM          & Standard Model \\
%          CC          & Charge Current Interaction \\
%          NC          & Neutral Current Interaction \\
%          VEV         & Vacuum Expectation Value \\
%          PMNS        & Pontecorvo Maki Nakagawa Sakata Matrix \\
%$0\nu\nu\beta\beta$   & Neutrinoless Double Beta Decay \\
%          SSM         & Standard Solar Model \\
%          SK          & Super-Kamiokande Experiment \\
%          DAR         & Decay at Rest \\
%           DIF         & Decay in Flight \\
%           IBD         & Inverse Beta Decay \\
%           UHE         & Ultra High Energy \\
%           AGN         & Active Galactic Nuclei \\
%           GRB         & Gamma Ray Burst \\
%           GUT         & Grand Unified Theories \\
%           LEP         & Large Electron-Positron collider \\
%           OMSD        & One Mass Scale Dominance Approximation \\
%           MSW         & Mikheyev Smirnov Wolfenstein Effect \\
%           PREM        & Preliminary Reference Earth Model \\
%           GLoBES      & General Long-Baseline Experiment Simulator \\
%           NH          & Normal Hierarchy \\
%           IH          & Inverted Hierarchy \\
%            QD          & Quasi Degenerate \\
            LO          & Lower Octant \\
            HO          & Higher Octant \\
            LHP         & Lower Half-Plane of $\dcp$ \\
            UHP         & Upper Half-Plane of $\dcp$ \\
            T2K         & Tokai to Kamioka \\
            POT         & Protons on Target \\
            \nova\      & NuMI Off-axis $\nu_e$ Appearance \\
            LAGUNA      & Large Apparatus studying Grand Unification and \\
                        &  Neutrino Astrophysics \\
            LBNO        & Long-Baseline Neutrino Oscillation Experiment\\
            LBNE        & Long-Baseline Neutrino Experiment \\
            LArTPC      & Liquid Argon Time Projection Chamber \\
            SURF        & Sanford Underground Research Facility \\
            DUNE        & Deep Underground Neutrino Experiment \\
            INO         & India-based Neutrino Observatory \\
            ICAL        & Iron Calorimeter Detector \\
            LBL         & Long Baseline Experiments \\
            CPV         & CP Violation \\
            TASD        & Totally Active Scintillator Detector \\
            ND          & Near Detector \\
            FD          & Far Detector \\
            TBM         & Tri-bimaximal Mixing \\
            SBL         & Short Baseline Experiments \\
          
         
    \end{tabular}
    \end{center}
\end{table}






==> publications.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                 List of Publications                %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
{\Large \textbf{LIST OF PUBLICATIONS}}
\end{center}
\vspace{0.5cm}

{\large{\bf Publications contributing to this thesis :}}

\begin{enumerate}

       \item {\it Two Zero Mass Matrices and Sterile Neutrinos}, \\
                  {\bf M.~Ghosh}, S.~Goswami and S.~Gupta, 
                  JHEP {\bf 1304}, 103 (2013).

       \item {\it Implication of a vanishing element in the 3+1 scenario}, \\
                  {\bf M.~Ghosh}, S.~Goswami, S.~Gupta and C.~S.~Kim, 
                  Phys.\ Rev.\ D {\bf 88}, no. 3, 033009 (2013).


       \item {\it Can atmospheric neutrino experiments provide the first hint of leptonic CP violation?}, \\
                  {\bf M.~Ghosh}, P.~Ghoshal, S.~Goswami and S.~K.~Raut, 
                  Phys.\ Rev.\ D {\bf 89}, no. 1, 011301 (2014).
                  
        \item {\it Synergies between neutrino oscillation experiments: an 'adequate` configuration for LBNO}, \\
                  {\bf M.~Ghosh}, P.~Ghoshal, S.~Goswami and S.~K.~Raut, 
                  JHEP {\bf 1403}, 094 (2014).

       \item {\it Probing CP violation with the first three years of ultrahigh energy neutrinos from IceCube}, \\
                   A.~Chatterjee, M.~M.~Devi, {\bf M.~Ghosh}, R.~Moharana and S.~K.~Raut, 
                   Phys.\ Rev.\ D {\bf 90}, no. 7, 073003 (2014).


       \item {\it Evidence for leptonic CP phase from NO$\nu$A, T2K and ICAL: A chronological progression}, \\
                  {\bf M.~Ghosh}, P.~Ghoshal, S.~Goswami and S.~K.~Raut, 
                  Nucl.\ Phys.\ B {\bf 884}, 274 (2014).      
                  
       \item {\it Economizing the LBNE configuration with current experiments}, \\
                   {\bf M.~Ghosh}, S.~Goswami and S.~K.~Raut, 
                  arXiv:1412.1744 [hep-ph] (communicated for publication).          


\end{enumerate}

{\large{\bf Other publications :}}

\begin{enumerate}
 \item {\it Can the hint of $\delta_{CP}$ from T2K also indicate the hierarchy and octant?}, \\
                  {\bf M.~Ghosh}, S.~Goswami and S.~K.~Raut, 
                  arXiv:1409.5046 [hep-ph]  (communicated for publication).
                  
 \item {\it Identifying and resolving the degeneracies in neutrino oscillation parameters in current experiments}, \\
                 {\bf M.~Ghosh}, P.~Ghoshal, S.~Goswami, N.~Nath and S.~K.~Raut,
                 arXiv:1504.06283 [hep-ph] (communicated for publication). 
\end{enumerate}


